Parameterized and approximation algorithms for coverings points with segments in the plane

We study parameterized and approximation algorithms for a variant of Set Cover, where the universe of elements to be covered consists of points in the plane and the sets with which the points should be covered are segments. We call this problem Segment Set Cover. We also consider a relaxation of the problem called $\delta$-extension, where we need to cover the points by segments that are extended by a tiny fraction, but we compare the solution's quality to the optimum without extension. For the unparameterized variant, we prove that Segment Set Cover does not admit a PTAS unless $\mathsf{P}=\mathsf{NP}$, even if we restrict segments to be axis-parallel and allow $\frac{1}{2}$-extension. On the other hand, we show that parameterization helps for the tractability of Segment Set Cover: we give an FPT algorithm for unweighted Segment Set Cover parameterized by the solution size $k$, a parameterized approximation scheme for Weighted Segment Set Cover with $k$ being the parameter, and an FPT algorithm for Weighted Segment Set Cover with $\delta$-extension parameterized by $k$ and $\delta$. In the last two results, relaxing the problem is probably necessary: we prove that Weighted Segment Set Cover without any relaxation is $\mathsf{W}[1]$-hard and, assuming ETH, there does not exist an algorithm running in time $f(k)\cdot n^{o(k / \log k)}$. This holds even if one restricts attention to axis-parallel segments.

==> figures/diag_definition.tex <==
	
\definecolor{guards_color}{RGB}{80, 120, 255}

{\tikzset{guard_h/.style={
    circle, draw=guards_color, fill, fill=guards_color, minimum size=2pt,inner sep=0pt, outer sep=0pt,
    prefix after command= {\pgfextra{\tikzset{every
    label/.style={label distance=0.1cm,rotate=90,text=guards_color,font=\footnotesize}}}}
    }
}
{\tikzset{node_h/.style={
    circle, draw=black, fill, fill=black, minimum size=4pt,inner sep=0pt, outer sep=0pt,
    prefix after command= {\pgfextra{\tikzset{every
    label/.style={label distance=0.1cm,rotate=90,text=black}}}}
    }
}
{\tikzset{guard_v/.style={
    circle, draw=guards_color, fill, fill=guards_color, minimum size=2pt,inner sep=0pt, outer sep=0pt,
    prefix after command= {\pgfextra{\tikzset{every
    label/.style={label distance=0.1cm,text=guards_color,font=\footnotesize}}}}
    }
}
{\tikzset{node_v/.style={
    circle, draw=black, fill, fill=black, minimum size=4pt,inner sep=0pt, outer sep=0pt,
    prefix after command= {\pgfextra{\tikzset{every
    label/.style={label distance=0.1cm,text=black}}}}
    }
}

\newcommand{\addNodeV}[2]{
	\node[guard_v, label={left:$v_{i,j,#2}^D$}] at (0, \l#1) {};
	\node[node_v, label={left:$v_{i,j,#2}$}] at (0,\x#1) {};
	\node[guard_v, label={left:$v_{i,j,#2}^U$}] at (0, \r#1) {};
}

\newcommand{\addNodeH}[2]{
	\node[guard_h, label={left:$h_{i,j,#2}^L$}] at (\l#1,0) {};
	\node[node_h, label={left:$h_{i,j,#2}$}] at (\x#1,0) {};
	\node[guard_h, label={left:$h_{i,j,#2}^R$}] at (\r#1,0) {};
}

\begin{figure}
\begin{center}
\begin{tikzpicture}[main/.style = {draw, circle}]
\tikzmath{
	\step=2;
	\eps=0.5;
	\x1=\step;
	\x2=\x1+\step;
	\x3=\x2+\step;
	\x4=\x3+\step;
	\x5=\x4+\step;
	\x6=\x5+\step;
	\l1=\x1-\eps;
	\r1=\x1+\eps;
	\l2=\x2-\eps;
	\r2=\x2+\eps;
	\l3=\x3-\eps;
	\r3=\x3+\eps;
	\l4=\x4-\eps;
	\r4=\x4+\eps;
	\l5=\x5-\eps;
	\r5=\x5+\eps;
	\l6=\x6-\eps;
	\r6=\x6+\eps;
}

\draw (0,\x1) -- (\x1,0) node[midway, above] {$\delta$};
\draw (0,\x2) -- (\x2,0) node[midway, above] {$\delta$};
\draw (0,\x3) -- (\x3,0) node[midway, above] {$\delta$};
\draw (0,\x5) -- (\x5,0) node[midway, above] {$\delta$};
\draw (0,\x6) -- (\x6,0) node[midway, above] {$\delta$};

\addNodeV{1}{1}
\addNodeV{2}{2}
\addNodeV{3}{3}
\filldraw[black] (0,\x4) circle (0pt) node[anchor=east] {$\ldots$};
\addNodeV{5}{n^2-1}
\addNodeV{6}{n^2}

\addNodeH{1}{1}
\addNodeH{2}{2}
\addNodeH{3}{3}
\filldraw[black] (\x4,0) circle (0pt) node[anchor=north] {$\ldots$};
\addNodeH{5}{n^2-1}
\addNodeH{6}{n^2}
\end{tikzpicture} 
\end{center}
\caption{\textbf{Vertices and segments in $\alldiag$.}}
This is an example of constructed points any $1 \le i,j \le k$.
Points from $H$ and $V$ are marked in black,
their guards are marked in \textcolor{guards_color}{blue}.
You can also see segments from $\alldiag$ with their weights (equal to $\delta$).
\label{fig:diag_def}
\end{figure}


==> figures/grid_tiling_example.tex <==
\definecolor{alternative_sol}{RGB}{48, 48, 255}
\definecolor{bad_sol}{RGB}{255, 48, 48}

\begin{figure}[h]
\begin{center}
\begin{tabular}{ c|c|c|c|c| } 
          & $x(1)=3$ & $x(2)=1$ & $x(3)=3$ & $x(4) = 7$\\ 
 \hline
 $y(4)=1$
	& \makecell{$\textcolor{alternative_sol}{(2,1)};(2,2);$\\$\textbf{(3,1)};(3,9)$}
	& $\textbf{(1,1)}; (3,1)$
	& $\textbf{(3,1)}; (7,2)$
	& $\textcolor{bad_sol}{(2,1)}; \textbf{(7,1)}$\\ 
 \hline
 $y(3)=1$
	& \makecell{$\textcolor{alternative_sol}{(2,1)};\textbf{(3,1)};$\\$(4,2);(8,2)$}
	& $\textbf{(1,1)}; (1,3)$
	& $\textbf{(3,1)}; (4,3)$
	& $\textcolor{bad_sol}{\textbf{(2,2)}}; \textbf{(7,1)}$\\ 
 \hline
 $y(2)=6$
	& $\textcolor{alternative_sol}{(2,6)};\textbf{(3,6)}$
	& \makecell{$(1,2); \textbf{(1,6)};$\\$(2,6)$}
	& $(2,6); \textbf{(3,6)}$
	& $\textcolor{bad_sol}{(2,6)};\textbf{(7,6)}$\\ 
 \hline
 $y(1)=4$
	& \makecell{$\textcolor{alternative_sol}{(2,4)};(2,6);$\\$\textbf{(3,4)};\textcolor{bad_sol}{(3,9)}$}
	& $\textbf{(1,4)}; \textcolor{bad_sol}{(1,9)}$
	& $\textbf{(3,4)}; \textcolor{bad_sol}{(3,9)}$
	& $\textcolor{bad_sol}{(2,9)}; \textbf{(7,4)}$\\ 
 \hline
\end{tabular}
\end{center}
\caption{\textbf{Example of a $\GridTiling$ instance and its solution.}}
In the first row and column of the table you can see the solution:
functions $x$ and $y$.
The~tiles used in this solution are marked in \textbf{bold}.
If we instead chose the tiles marked in \textcolor{alternative_sol}{blue}
(whenever there is one, taking the tile marked in \textbf{bold} otherwise),
then that corresponds to setting $x(1)=2$, and would also form a correct solution.
On the other hand, if we instead chose the tiles marked in \textcolor{bad_sol}{red}
(as before), then this corresponds to setting ${y(1)=9}$ and $x(4)=2$
and that would $\textbf{not}$ form a correct solution.
Even though the first row is correct,
the cell with coordinates (3,4) requires tile (2,1), not (2,2)
(marked in \textbf{\textcolor{bad_sol}{bold red}}).
\label{fig:grid_tiling_exmample}
\end{figure}


==> figures/w1_hard_segments.tex <==

\definecolor{beg_color}{RGB}{255, 40, 40}
\definecolor{seg_color1}{RGB}{40, 40, 255}
\definecolor{seg_color2}{RGB}{40, 150, 40}

\newcommand{\addNode}[4]{
	\node[guard_h, label={left:$h_{#1,j,t_{#2,#3}}^L$}] at (\l#4,0) {};
	\node[node_h, label={left:$h_{#1,j,t_{#2,#3}}$}] at (\x#4,0) {};
	\node[guard_h, label={left:$h_{#1,j,t_{#2,#3}}^R$}] at (\r#4,0) {};
}

\begin{figure}
\hspace*{-1.5cm}
\begin{tikzpicture}[main/.style = {draw, circle}]
\tikzmath{
\step=2;
\eps=0.5;
%genereted by gen_math.py
\x1=\step;
\x2=\x1+\step;
\x3=\x2+\step;
\x4=\x3+\step;
\x5=\x4+\step;
\x6=\x5+\step;
\x7=\x6+\step;
\x8=\x7+\step;
\x9=\x8+\step;
\l1=\x1-\eps;
\r1=\x1+\eps;
\l2=\x2-\eps;
\r2=\x2+\eps;
\l3=\x3-\eps;
\r3=\x3+\eps;
\l4=\x4-\eps;
\r4=\x4+\eps;
\l5=\x5-\eps;
\r5=\x5+\eps;
\l6=\x6-\eps;
\r6=\x6+\eps;
\l7=\x7-\eps;
\r7=\x7+\eps;
\l8=\x8-\eps;
\r8=\x8+\eps;
\l9=\x9-\eps;
\r9=\x9+\eps;
}

\draw [beg_color] (\l1,0) to[out=150,in=30, looseness=200] (1.49,0);
\draw [beg_color] (\l1,0) to[out=40,in=140] (\l2,0);
\draw [beg_color] (\l1,0) to[out=40,in=140] (\l3,0);
\draw [beg_color] (\l1,0) to[out=40,in=140] (\l4,0);


\draw [seg_color1] (\r1,0) to[out=20,in=160] (\l6,0);
\draw [seg_color1] (\r1,0) to[out=20,in=160] (\l8,0);
\draw [seg_color2] (\r2,0) to[out=20,in=160] (\l7,0);
\draw [seg_color2] (\r2,0) to[out=20,in=160] (\l9,0);
\draw [seg_color1] (\r3,0) to[out=20,in=160] (\l6,0);
\draw [seg_color1] (\r3,0) to[out=20,in=160] (\l8,0);
\draw [seg_color2] (\r4,0) to[out=20,in=160] (\l7,0);
\draw [seg_color2] (\r4,0) to[out=20,in=160] (\l9,0);

\addNode{1}{1}{1}{1}
\addNode{1}{1}{2}{2}
\addNode{1}{2}{1}{3}
\addNode{1}{2}{2}{4}
\addNode{2}{1}{1}{6}
\addNode{2}{1}{2}{7}
\addNode{2}{2}{1}{8}
\addNode{2}{2}{2}{9}

\end{tikzpicture} 
\caption{\textbf{Vertices and segments in $HOR$.}}
This is an example for $n=2$ and any $1 \le j \le k$.
Points from $H$ are marked in black, their guards are marked in \textcolor{guards_color}{light blue}.
$t_{i,j}$ is a notation that we use for $\order^{-1}(i,j)$.
Segments are represented as arcs between endpoints.
You can see $\horbeg{j}{t}$ segments in \textcolor{beg_color}{red}.
$\horbeg{j}{1}$ is degenerated to a single point at $h_{1,1,t_{1,1}}^L$.
Segments $\hor{i}{j}{t_{x_1,y}}{t_{x_2,y}}$
are marked in \textcolor{seg_color1}{blue} and \textcolor{seg_color2}{green}.
\textcolor{seg_color1}{Blue} segments connect $t_{x_1,y}$ and $t_{x_2,y}$
such that they share y-coordinate equal to 1,
for~\textcolor{seg_color2}{green} segments it is equal to 2.

\label{fig:segments_def}
\end{figure}


==> fpt_weighted_segments.tex <==
\subsection{Weighted segments with $\delta$-extension}
\label{section:fpt_weighted}

In this section we prove Theorem~\ref{fpt_weighted_segment}, restated below for convenience. 

\fptWeightedSegment*

%Recall that some relaxation of the $\WeightedSegmentSetCover$ problem is probably necessary to obtain fixed-parameter tractability: in Section~\ref{chapter:w1_hard} we will show that without any relaxation, the problem is W[1]-hard. Here, we show that the $\delta$-extension relaxation leads to fixed-parameter tractability.

Roughly speaking, our approach to prove Theorem~\ref{fpt_weighted_segment} is to find a small kernel for the problem; but we need to be careful with the definition of kernelization, because we work in the $\delta$-extension model. The key technical tool will be the notion of a {\em{dense subset}}.

\subparagraph*{Dense subsets.}
Intuitively speaking, for a set of collinear points $C$, a subset $A\subseteq C$ is dense if any small cover of $A$ becomes a cover of $C$ after a tiny extension. This is formalized in the following definition.

\begin{definition}
	For a set of collinear points $C$,
	a subset $A \subseteq C$ is {\em{$(k,\delta)$-dense}} in $C$ 
	if for any set of segments $\Rr$ that covers $A$ and
	such that $|\Rr| \le k$, it holds that $\Rr^{+\delta}$ covers $C$.
\end{definition}

The key combinatorial observation in our approach is expressed in the following Lemma~\ref{dense_set_exists}: in every collinear set $C$ one can always find a $(k,\delta)$-dense subset of size bounded by a function of $k$ and $\delta$.
Later, this lemma will allow us to find a kernel
for our original problem.

\begin{lemma}
	\label{dense_set_exists}
	For every set $C$ of collinear points in the plane, $\delta > 0$ and $k \ge 1$,
	there exists a $(k,\delta)$-dense set $A \subseteq C$ of size
	at most $(2+\frac{4}{\delta})^k$.
	Moreover, such a $(k,\delta)$-dense set
	can be computed in time $\Oh(|C| \cdot (2+\frac{4}{\delta})^k)$.
\end{lemma}

\begin{proof}
We give a proof of the existence of such a dense subset $A$, and at the end we will argue that the proof naturally gives rise to an algorithm with the promised complexity. We fix $\delta$ and proceed by induction on $k$. Formally, we shall prove the following stronger statement:
For any set of collinear points $C$, there exists a subset $A\subseteq C$ such that:
\begin{itemize}
\item $A$ is $(k, \delta)$-dense in $C$,
\item $|A| \le (2+\frac{4}{\delta})^k$, and
\item the extreme points of $C$ are in $A$.
\end{itemize}

Consider first the base case when $k=1$.
Then it is sufficient to just take $A$ that consists of the (at most $2$) extreme points of $C$.
Indeed, if the extreme points of $C$ are covered with one segment, then this segment must cover the whole set $C$ (even without extension).
Thus, the set $A$ has size at most $2 < (2+\frac{4}{\delta})^1$, as required.

We now proceed to the inductive step.
Assuming inductive hypothesis for any set of collinear points $C$
and for parameter $k$, we will prove it for $k+1$.

Let $s$ be the minimal segment that includes all points from $C$.
That is, $s$ is the segment whose endpoints are the extreme points of $C$.

Split $s$ into $M \coloneqq \lceil1+\frac{4}{\delta}\rceil$ subsegments of equal length.
We name these segments $v_1,v_2,\ldots,v_M$ in order, and we consider them closed. Note that
$|v_i| = \frac{|s|}{M}$ for each $1 \le i \le M$, where $|\cdot|$ denotes the length of a segment.

Let $C_i$ be the subset of $C$ consisting of points belonging to $v_i$.
Further, let $t_i$ be the segment with endpoints being the extreme points of $C_i$.
Note that $t_i$ might be a degenerate single-point segment if $C_i$ consists of one point,
or even $t_i$ might be empty if $C_i$ is empty.
Figure~\ref{fig:fpt_v_f_def} presents an example of the construction.

\begin{figure}[h]
\begin{center}
\def\svgwidth{\textwidth}
\input{fpt_v_t_def.pdf_tex}
\caption{Example of the construction in the proof of Lemma~\ref{dense_set_exists} for $M = 7$ and some set of points $C$ (marked with black circles).
The top panel shows segments $v_i$. The middle panel shows segments~$t_i$. Note that $t_5$ is an empty segment,
because there are no points in $C$ that belong to $v_5$, while
each of the segments $t_3$ and $t_7$ is degenerated to a single point:
$c$ and $d$, respectively.
Segments $t_1$ and $t_2$ share one point $b$.
The bottom panel shows an example of the second case in the correctness proof: a solution $\Rr$ of size $4$ whose all segments intersect $t_4$. Then one of $y$ and $z$ will cover the whole of $C_4$ after extension.
}
\label{fig:fpt_v_f_def}
\end{center}
\end{figure}

We use the inductive hypothesis to choose a $(k, \delta)$-dense subset $A_i$ of $C_i$, for each $i\in \{1,\ldots,M\}$. Note that if $|C_i| \le 1$, then $A_i = C_i$, so $A_i$ is $(k, \delta)$-dense set for $C_i$. Also, by assumption, $A_i$ contains the extreme points of $C_i$.

Next, we define $A \coloneqq \bigcup_{i=1}^{M} A_i$.
Thus $A$ includes the extreme points of $C$,
because they are included in the sets $A_1$ and $A_M$.

By induction, the size of each $A_i$ is at most $(2+\frac{4}{\delta})^{k}$. Therefore,
$$|A|\leq M\left(2+\frac{4}{\delta}\right)^{k} =
\left\lceil1+\frac{4}{\delta}\right\rceil\cdot\left(2+\frac{4}{\delta}\right)^{k}
\le \left(2+\frac{4}{\delta}\right)^{k+1}.$$
We are left with verifying that $A$ is $(k+1,\delta)$-dense in $C$.
For this, consider any cover of $A$ with $k+1$ segments and call it $\Rr$.

Consider any segment $t_i$. If there exists a segment $x\in \Rr$ 
that is disjoint with $t_i$,
then $\Rr- \{x\}$ constitutes a cover of $A_i$ with at most $k$
segments.
Since $A_i$ is $(k, \delta)$-dense in $C_i$,
$(\Rr - \{x\})^{+\delta}$ covers $C_i$.
So $\Rr^{+\delta}$ covers $C_i$ as well.

On the other hand, if for any fixed $t_i$ a segment $x\in \Rr$ as above
does not exist, then all the $k+1$ segments of $\Rr$ intersect $t_i$.
An example of such a situation is depicted in the bottom panel of Figure~\ref{fig:fpt_v_f_def}.
Let us consider any such $t_i$.
By induction, the endpoints of $s$ are
in $A_1$ and $A_M$ respectively, so $\Rr$ must cover them.
So for each endpoint of $s$, there exists
a segment in $\Rr$ that contains this endpoint and intersects $t_i$.
Let us call these two segments $y$ and~$z$. It follows that
$|y| + |z| + |t_i| \ge |s|$.
Since $|t_i| \le |v_i| = \frac{|s|}{M} \le \frac{|s|}{1+\frac{4}{\delta}} = \frac{\delta|s|}{\delta+4}$,
we have $$\max(|y|, |z|) \ge |s|\left(1-\frac{\delta}{\delta+4}\right)/2 = \frac{2|s|}{\delta+4}.$$
% 
% \begin{figure}[h]
% \begin{center}
% \def\svgwidth{\columnwidth}
% \input{fpt_tricky_case.pdf_tex}
% \end{center}
% \caption{Example of all $k+1$ segments intersecting one segment $t_i$.
% The top panel shows segments $t_i$ from the example from Figure~\ref{fig:fpt_v_f_def}.
% The bottom panel shows a solution $\Rr$ of size $4$ whose all segments intersect $t_4$. Then one of $y$ and $z$ will cover the whole of $C_4$ after extension.}
% \label{fig:fpt_tricky_case}
% \end{figure}
After $\delta$-extension, the longer of the segments $y$ and $z$ will
expand at both ends by at least:
$$\delta/2\cdot \max(|y|, |z|) \ge \frac{\delta|s|}{\delta+4} =
\frac{|s|}{1+\frac{4}{\delta}} \ge \frac{|s|}{M} = |v_i| \ge |t_i|.$$
Therefore, the longer of segments $y$ and $z$ will cover the whole segment $t_i$
after $\delta$-extension. We conclude that $\Rr^{+\delta}$ covers $C_i$ as well.

Since $C = \bigcup_{i=1}^M C_i$, we conclude that $\Rr^{+\delta}$ covers $C$. So indeed, $A$ is $(k+1,\delta)$-dense in~$C$. This concludes the proof of the existence of such a dense set $A$. To compute $A$ in time $\Oh\left(|C|\cdot\left(2+\frac{4}{\delta}\right)^k\right)$ observe that the inductive proof explained above can be easily turned into a recursive procedure that for a given $C$ and $k$, outputs a $(k,\delta)$-dense subset of $C$. The recursion tree of this procedure has size $\Oh\left(\left(2+\frac{4}{\delta}\right)^k\right)$ in total, while every recursive calls uses $\Oh(|C|)$ time for internal computation, so the total running time is $\Oh\left(|C|\cdot\left(2+\frac{4}{\delta}\right)^k\right)$.
\end{proof}

\subparagraph*{Long lines.} We need a few additional observations in the spirit of the algorithm of Theorem~\ref{thm:few_weights}. For a finite set of points $\points$ in the plane, call a line $L$ {\em{$k$-long}} with respect to $\points$ if $L$ contains more than $k$ points from $\points$. We have the following observations.

\begin{lemma}
\label{few_long_lines}
Let $\points$ be a finite set of points in the plane such that there are more than $k$ lines that are $k$-long with respect to $\points$. Then 
$\points$ cannot be covered with $k$ segments.
\end{lemma}
\begin{proof}
We proceed by contradiction.
Assume there are at least $k+1$ different
$k$-long lines and there is a set of segments $\Rr$ of size at most $k$
covering all points in $\points$.

Consider any $k$-long line $L$.
Note that every segment $\Rr$ which is not collinear with~$L$,
covers at most one point that lies on $L$.
Since $L$ is long, there are at least $k+1$ points from $\points$ that lie on $L$.
This implies that there must be a segment in $\Rr$ that is
collinear with~$L$.

Since we have at least $k+1$ different long lines,
there are at least $k+1$
segments in $\Rr$ collinear with different lines.
This contradicts the assumption that $|\Rr| \le k$.
\end{proof}

\begin{lemma}
\label{few_points}
Let $\points$ be a finite set of points in the plane such that there are more than $k^2$ points from $\points$
that do not lie on any line that is $k$-long with respect to $\points$. Then $\points$ cannot be covered with $k$ segments.
\end{lemma}
\begin{proof}
We proceed by contradiction.
Assume that we have more than $k^2$ points
in $\points$ that do not lie on any $k$-long line. Call this set $A$.
Suppose there is a set of segments $\Rr$ of size at most $k$
that covers all points in $\points$.

Since any line in the plane can cover only at most $k$ points in $A$, the same is also true for every segment in $\Rr$. Therefore, the segments from $\Rr$ can cover at most $k^2$ points in $A$ in total. As $|A|>k^2$, $\Rr$ cannot cover the whole $A$, which is a subset of $\points$; a contradiction.
\end{proof}

We are now ready to give a proof of Theorem \ref{fpt_weighted_segment}.

\newcommand{\instance}{(\points,\sets,\mathbf{w})}
\newcommand{\instancePrim}{(\points',\sets',\mathbf{w})}

\begin{proof}[Proof of Theorem \ref{fpt_weighted_segment}]
Let $\instance$ be the input instance of $\WeightedSegmentSetCover$, where $\mathbf{w}\colon \sets\to \mathbb{R}_{\geq 0}$ is the weight function. Further, let $k$ and $\delta>0$ be the input parameters.
Our goal is to either conclude that $\instance$ has no solution of cardinality at most $k$, or to find an instance
$\instancePrim$ of size bounded by $f(k,\delta)$ for some computable function $f$ and satisfying $\points'\subseteq \points$ and $\sets'\subseteq \sets$, such that the following two properties hold:
\begin{itemize}
\item \textit{(Property 1)} For every set $\sol\subseteq \sets$ such that $|\sol|\leq k$ and $\sol$ covers $\points$,
there is a set $\sol_1 \subseteq \sets'$ such that
$|\sol_1| \le k$, the weight of $\sol_1$ is not greater than the weight of $\sol$,
and $\sol_1$ covers $\points'$.
\item \textit{(Property 2)}
For every set $\sol \subseteq \sets'$ such that $|\sol| \le k$
and $\sol$ covers all points in $\points'$, $\sol^{+\delta}$
covers all points in the original set $\points$.
\end{itemize}
Suppose we constructed such an instance $\instancePrim$.
Then using \textit{Property 1} we know that an optimum solution 
of size at most $k$ to $\instancePrim$
has no greater weight than an optimum solution
of size at most $k$ to $\instance$.
On the other hand, using \textit{Property 2} we know that
any solution to $\instancePrim$
after $\delta$-extension covers $\points$. So it will remain to find an optimum solution to the instance $\instancePrim$. This can be done by brute-force in time $|\sets'|^{k+\Oh(1)}\cdot |\points'|^{\Oh(1)}$, which is bounded by a computable function of $k$ and $\delta$.

% Therefore, finding such sets 
% and solving the instance $\instancePrim$
% by iterating over all of the subsets of $\sets'$
% of size at most $k$
% in desired complexity
% is sufficient to prove Theorem \ref{fpt_weighted_segment}.

It remains to construct the instance $\instancePrim$.
Let $\ell$ be the number of different lines that are $k$-long with respect to $\points$.
By Lemmas~\ref{few_long_lines} and~\ref{few_points},
if we had more than $k$ different $k$-long lines
or more than $k^2$ points from $\points$
that do not lie on any $k$-long line, then we can safely conclude that $(\points,\sets,\mathbf{w})$ has no solution of cardinality at most $k$, and terminate the algorithm. So assume otherwise, in particular $\ell\leq k$.

Next, we cover $\points$ with at most $k+1$ sets:
\begin{itemize}
\item $D$ consists of all points in $\points$ that do not lie on any $k$-long line. Then we have $|D| \le k^2$.
\item For $1 \le i \le \ell$, $C_i$ consists of all points in $\points$ that lie on the $i$-th long line. Then $|C_i| > k$.
\end{itemize}
Note that sets $C_i$ do not need to be disjoint.

For every set $C_i$, we apply Lemma~\ref{dense_set_exists}
to obtain a subset $A_i\subseteq C_i$ that is $(k,\delta)$-dense and satisfies $|A_i| \le (2+\frac{4}{\delta})^k$.
We define $\points'\coloneqq D \cup \bigcup_{i=1}^\ell A_i$. Thus, $\points'$ has size at most
$k^2 + k(2+\frac{4}{\delta})^k$.
Further, we define $\sets'$ as follows: for every pair of points in $\points'$, if there are segments in $\sets$ that cover this pair of points, 
we choose one such segment with the lowest weight and include it in $\sets'$.
Thus $\sets'$ has size at most $|\points'|^2$,
which means that both $\sets'$ and $\points'$ have sizes bounded
by~$\Oh\left((k^2 + k(2+\frac{4}{\delta})^k)^2\right)$. We are left with verifying Properties 1 and~2.

For Property~2, consider any set $\sol \subseteq \sets'$ such that $|\sol| \le k$
and $\sol$ covers all points in $\points'$. Then in particular, for every $i\in \{1,\ldots,\ell\}$, $\sol$ in covers all points in $A_i$. As $A_i$ is $(k,\delta)$-dense in $C_i$, we conclude that $\sol^{+\delta}$ covers $C_i$. Hence $\sol^{+\delta}$ covers $D\cup \bigcup_{i=1}^\ell C_i=\points$, as required.

For Property~1, consider any solution
$\sol$ to $\instance$ of size at most $k$.
For every segment $s\in \sol$, let $B_s$ be the set of points in $\points'$ that are covered by $s$.
$B_s$ is of course a set of collinear points, hence
$B_s$ can be covered by any segment that covers the extreme points of~$B_s$.
Therefore, we can replace $s$ with a segment $s'\in \sets$
that has the lowest weight among the segments that cover the extreme points of~$B_s$.
Such a segment belongs to $\sets'$ by construction, and $s'$ has weight no greater than the weight of $s$, because $s$ also covers the extreme points of $B_s$. Therefore, if $\sol_1\subseteq \sets'$ is the set obtained by performing such replacement for every $s\in \sol$, then $\sol_1$ has both size and weight not greater than $\sol$, and $\sol_1$ covers $\points'$.
\end{proof}


